Window Token Concatenation for Efficient Visual Large Language Models

To effectively reduce the visual tokens in Visual Large Language Models (VLLMs), we propose a novel approach called Window Token Concatenation (WiCo). Specifically, we employ a sliding window to concatenate spatially adjacent visual tokens. However, directly concatenating these tokens may group diverse tokens into one, and thus obscure some fine details. To address this challenge, we propose fine-tuning the last few layers of the vision encoder to adaptively adjust the visual tokens, encouraging that those within the same window exhibit similar features. To further enhance the performance on fine-grained visual understanding tasks, we introduce WiCo+, which decomposes the visual tokens in later layers of the LLM. Such a design enjoys the merits of the large perception field of the LLM for fine-grained visual understanding while keeping a small number of visual tokens for efficient inference. We perform extensive experiments on both coarse- and fine-grained visual understanding tasks based on LLaVA-1.5 and Shikra, showing better performance compared with existing token reduction projectors. The code is available: https://github.com/JackYFL/WiCo.

==> tables/conv_wico.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|cccccc}
        \toprule
         Methods & VQA\textsuperscript{v2} & SQA\textsuperscript{I} & VQA\textsuperscript{T} & POPE & MME & MMB  \\
         \midrule
         WiCo (convolution) & 76.2 & 69.7 & 53.2 & 84.9 & 1409.1 & 63.2 \\
         \rowcolor{purple!15} WiCo (self-attention) & 76.7 & 68.4 & 54.7 & 85.1 & 1435.4 & 64.5 \\
         \bottomrule
    \end{tabular}
    }
    \caption{Influence of the pre-merging technique of WiCo for LLaVA-1.5 on six benchmarks.}
    \label{tab:conv_wico}
\end{table}

==> tables/selfatt_position.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c|cccccc}
        \toprule
         Methods & VQA\textsuperscript{v2} & SQA\textsuperscript{I} & VQA\textsuperscript{T} & POPE & MME & MMB  \\
         \midrule
         WiCo (self-attention after concatenation) & 74.9 & 68.8 & 51.4 & 84.5 & 1361.2 & 62.1 \\
         \rowcolor{purple!15} WiCo (self-attention before concatenation) & 76.7 & 68.4 & 54.7 & 85.1 & 1435.4 & 64.5 \\
         \bottomrule
    \end{tabular}
    }
    \caption{Influence of the self-attention position of WiCo for LLaVA-1.5 on six benchmarks.}
    \label{tab:selfatt_pos}
\end{table}
